The Search for Thermonuclear Transients from the Tidal Disruption of a White Dwarf by an Intermediate Mass Black Hole

The close encounter of a white dwarf (WD) with a black hole (BH) could result in the tidal disruption of the WD. During this encounter, the WD can undergo a thermonuclear explosion due to its tidal compression, resulting in an optical transient similar to a Type Ia supernova (SN Ia), hereafter a Ia-TDE. Nevertheless, this will only be physically observable if the BH is $\lesssim 10^5$M$_\odot$. Finding a Ia-TDE would therefore imply the discovery of an intermediate mass black hole (IMBH) $\lesssim 10^5$ M$_\odot$. Here, we search the entire Zwicky Transient Facility (ZTF) alert stream for the elusive Ia-TDEs. We restrict our search to nuclear transients in dwarf galaxies, the likely sites for IMBHs, and find a total of six possible nuclear Ia-TDE candidates. We find SN\,2020lrt to be the most likely Ia-TDE candidate, thanks to its strong resemblance to light curve and spectroscopic models of Ia-TDEs. We measure the stellar masses of the dwarf galaxies hosting these transients to be $\lesssim 10^{9}$M$_\odot$; if confirmed to harbor BHs, these would prove the existence of IMBHs in some of the lowest-mass galaxies known. Additionally, we searched for off-nuclear Ia-TDEs, but were unable to find more robust candidates in the outskirts of galaxies than in their nuclei. This supports the hypothesis that the nuclear Ia-TDEs candidates are WDs tidally compressed by IMBHs in the cores of galaxies, as opposed to a class of transient that can happen anywhere in a galaxy. We have laid the groundwork to systematically search for Ia-TDE candidates in existing and future time-domain surveys. Rapid characterization of their nature will result in not only the confirmation of a Ia-TDE, but also the unambiguous discovery of bonafide IMBHs.

==> mycommands.tex <==
% New Commands
\newcommand{\tc}[2][red]{\textcolor{#1}{\emph{\textbf{#2}}}}
\newcommand{\ksmag}{\emph{Ks}~magnitudes }
\newcommand{\jmag}{\emph{J}~magnitudes }
\newcommand{\kpmags}{\emph{Kp}~magnitudes }
\newcommand{\kpmag}{\emph{Kp}~magnitude }
\newcommand{\teff}{\ensuremath{T_{\mathrm{eff}}}}
\newcommand{\logg}{\ensuremath{\log g}}
\newcommand{\kepler}{{\em Kepler}\xspace}
\def\msun{{\rm\,M_\odot}}
\def\rsun{{\rm\,R_\odot}}
\def\mearth{{\rm\,M_\oplus}}
\def\rearth{{\rm\,R_\oplus}}
\def\fearth{{\rm\,F_\oplus}}
\def\lsun{{\rm\,L_\odot}}
\newcommand{\hho}{H$_2$O}
\newcommand{\hh}{H$_2$}
\newcommand{\oo}{O$_2$}
\newcommand{\chhhh}{CH$_4$}
\newcommand{\mjup}{{\rm M}_{\rm Jup}}
\newcommand{\kms}{\rm km\ s^{-1}}
\newcommand{\mps}{\rm m\ s^{-1}}
\newcommand{\cspg}{\rm\ cm^2\ g^{-1}}
\newcommand{\ergs}{\rm\ erg\ s^{-1}}
\newcommand{\kelvin}{\rm K}
\newcommand{\angstrom}{\rm \AA}
\newcommand{\oneday}{\rm day}
\newcommand{\days}{\rm days}
\newcommand{\hours}{\rm hours}
\newcommand{\meter}{\rm m}
\newcommand{\HST}{{\it HST}}
\newcommand{\hubble}{{\it HST}}
\newcommand{\spitzer}{{\it Spitzer}}
\newcommand{\fermi}{{\it Fermi}}
\newcommand{\swift}{{\it Swift}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\mosfit}{{\tt MOSFiT}}
\newcommand{\zeroth}{$0^{\rm th}$}
\newcommand{\first}{$1^{st}$}
\newcommand{\second}{$2^{nd}$}
\newcommand{\third}{$3^{rd}$}
\newcommand{\fourth}{$4^{th}$}
\newcommand{\e}{${\rm e^{-}}$}
\newcommand{\persecond}{${\rm s^{-1}}$}
\newcommand{\perpixel}{${\rm pixel^{-1}}$}
\newcommand{\divideoot}{{\tt divide-oot}}
\newcommand{\modelramp}{{\tt model-ramp}}
\newcommand{\chisq}{$\chi^2$}
\newcommand{\calwf}{{\tt calwf3}}
\newcommand{\rp}{$R_{p}$}
\newcommand{\rs}{$R_{\star}$}
\newcommand{\flt}{{\tt flt}}
\definecolor{orange}{rgb}{.8,0.4,0}
\newcommand{\question}[1]{\sffamily {\em {\color{orange} [#1]}}\normalfont}
\newcommand{\todo}[1]{\sffamily {\em {\color{orange} #1}}\normalfont}
\newcommand{\mad}{\rm MAD}
\newcommand{\Mej}{M_{\rm ej}}
\newcommand{\vej}{v_{\rm ej}}
\newcommand{\apx}{\ensuremath{\sim}}
\newcommand{\WFDD}{{\tt WFDD}}
\newcommand{\WFDM}{{\tt WFDM}}
\newcommand{\WFDR}{{\tt WFDR}}

% Alternate Itemize
\newcommand{\outline}[1]{
\todo{\begin{itemize}
#1
\end{itemize}}}

% AutoRef Stuff
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}

\renewcommand*{\sectionautorefname}{Section} 
\renewcommand*{\subsectionautorefname}{Section} 

% Citation Alias
\defcitealias{LP98}{LP98}
\defcitealias{CowpBerger15}{CB15}

